Test Time Learning for Time Series Forecasting

Time-series forecasting has seen significant advancements with the introduction of token prediction mechanisms such as multi-head attention. However, these methods often struggle to achieve the same performance as in language modeling, primarily due to the quadratic computational cost and the complexity of capturing long-range dependencies in time-series data. State-space models (SSMs), such as Mamba, have shown promise in addressing these challenges by offering efficient solutions with linear RNNs capable of modeling long sequences with larger context windows. However, there remains room for improvement in accuracy and scalability. We propose the use of Test-Time Training (TTT) modules in a parallel architecture to enhance performance in long-term time series forecasting. Through extensive experiments on standard benchmark datasets, we demonstrate that TTT modules consistently outperform state-of-the-art models, including the Mamba-based TimeMachine, particularly in scenarios involving extended sequence and prediction lengths. Our results show significant improvements in Mean Squared Error (MSE) and Mean Absolute Error (MAE), especially on larger datasets such as Electricity, Traffic, and Weather, underscoring the effectiveness of TTT in capturing long-range dependencies. Additionally, we explore various convolutional architectures within the TTT framework, showing that even simple configurations like 1D convolution with small filters can achieve competitive results. This work sets a new benchmark for time-series forecasting and lays the groundwork for future research in scalable, high-performance forecasting models.

==> background.tex <==
\section{Background}
\textcolor{red}{PD: We do not need a separate section on background. You are not writing a thesis but a research paper. People know about attention, transformers. Structured State Space Models and Linear RNNs  should be discussed in Related Work (without the equations).}\\
\textbf{Maybe add 1 visualization.}

\subsection{Attention and Transformers for Sequential Data}

Transformer models, including iTransformer[], PatchTST[], and Crossformer[], have a strong capacity for capturing long-range dependencies, making them suitable for Long-Term Time Series Forecasting. However, they often face a challenge with quadratic complexity.

The Transformer architecture is a typical sequence-to-sequence (Seq2Seq) model that consists of an Encoder and a Decoder. The Encoder processes the input sequence and generates a context vector that contains the semantic information. The Decoder receives both the previous layer's output as the query ($Q$) and the encoder-generated context vector as keys ($K$) and values ($V$) to predict the next token. Both the Encoder and Decoder are composed of $N=6$ identical layers.

The core of the Transformer is the attention mechanism, which enables the model to focus on relationships between tokens at any positions within a sequence. However, traditional Recurrent Neural Networks (RNNs)[] are limited to capturing short-term local relationships.

A single attention head is known as Scaled Dot-Product Attention. The "Scaled" component refers to the inclusion of a scaling factor of $\frac{1}{\sqrt{d_k}}$. The attention function is calculated as follows:

\[
\text{Attention}(Q, K, V) = \text{softmax}\left(\frac{QK^T}{\sqrt{d_k}}\right)V
\]

where the dimensions of $Q$ and $K$ $\in \mathbb{R}^{n \times d_k}$, resulting in a complexity $O(n^2)$ that scales quadratically with sequence length $n$. This formula calculates the relationship between all pairs of tokens using queries, keys, and values.

Multi-Head Attention combines multiple attention heads, each focusing on different aspects of the queries. The outputs from these individual attention heads are concatenated and passed through a linear layer $W^O$.

\[
\text{MultiHead}(Q, K, V) = \text{Concat}(\text{head}_1, \dots, \text{head}_h)W^O
\]
where:
\[
\text{head}_i = \text{Attention}(QW_i^Q, KW_i^K, VW_i^V)
\]

The projections are parameter matrices:
\[
W_i^Q \in \mathbb{R}^{d_{\text{model}} \times d_k}, \quad W_i^K \in \mathbb{R}^{d_{\text{model}} \times d_k}, \quad W_i^V \in \mathbb{R}^{d_{\text{model}} \times d_v}
\]
\[
W^O \in \mathbb{R}^{h d_v \times d_{\text{model}}}
\]

As mentioned earlier, Transformer-based models can be computationally expensive when dealing with long context lengths, particularly in long-term time series forecasting.

\subsection{Structured State Space Models and Mamba}

Structured State Space Models (S4)~\cite{gu2022efficientlymodelinglongsequences}~\cite{gu2022parameterizationinitializationdiagonalstate}...~\cite{gupta2023simplifyingunderstandingstatespace} are a class of sequence models that use a hidden state vector to model input sequences. They are a great fit for long-term time-series forecasting (LTSF) due to their linear complexity and context-aware selectivity[].

S4 models are defined by four parameters: $(\Delta, A, B, C)$, where $\Delta$ represents the discretization step size of the SSM, $A$ is the state update matrix, and $B$ and $C$ are the input and output matrices, respectively. S4 models can be computed in two ways: using a linear recurrence or a global convolution.  The recurrent mode is used for autoregressive inference, while the convolutional mode allows for efficient parallelizable training

Similar to RNNs, the recurrent mode utilizes a hidden state vector to store historical information and updates it recursively.

$$h_t = \bar{A} h_{t-1} + \bar{B} x_t$$
$$y_t = C h_t$$

On the other hand, the convolutional mode transforms the recurrence formula into a convolutional operation, using the special structure of Toeplitz matrices. The computational efficiency of SSMs depends on the structure of the $A$ matrix. Commonly, it is designed to be diagonal, as is also used in Mamba.

$$\bar{K} = (C\bar{B}, C\bar{A}\bar{B}, \dots, C\bar{A}^k\bar{B}, \dots)$$
$$y = x * \bar{K}$$

In conclusion, Structured State Space Models effectively combine the advantages of CNNs and RNNs for efficient computation. However, they suffer from inherent time-invariance, making it challenging to perfectly process discrete data where selective memorization and forgetting of historical data are crucial. 

Mamba ~\cite{gu2024mambalineartimesequencemodeling}, on the other hand, addresses this problem by making the parameters $B$, $C$, and $\Delta$ functions of the input, using a Linear Layer or more complex MLP. 

In Mamba, we have $B_t = s_B(x_t) = \text{Linear}_N(x_t)$, where $B_t$ is the parameter $B$ 
 at time step $t$. $C_t = s_C(x_t) = \text{Linear}_N(x_t)$, where $C_t$ is the parameter $C$ at time step $t$. $\Delta_t = \tau_\Delta (\text{Parameter} + s_\Delta(x_t)) = \tau_\Delta (\text{Parameter} + \text{Broadcast}_D(\text{Linear}_1(x_t)))$. $\tau_\Delta = softplus$.

This modification allows the model to dynamically generate parameters that can be used for selectively filtering out irrelevant noise. Mamba's key feature is that it achieves Transformer-level performance while scaling linearly with time.


\subsection{Linear RNNs}
While Transformer-based architectures have recently dominated time series and sequence modeling tasks due to their ability to capture long-term dependencies, recurrent neural networks (RNNs) are still highly relevant for such tasks, particularly when handling long sequences efficiently. In ~\cite{orvieto2023resurrectingrecurrentneuralnetworks}, Deep Mind proposed Linear Recurrent Units (LRUs), a novel variant designed to address common challenges associated with traditional RNNs, such as vanishing and exploding gradients during backpropagation through time.

Linear Recurrent Units or Linear RNNs simplify the complex non-linear gating mechanisms found in typical RNNs, like LSTMs and GRUs, by incorporating linear state-space models. This modification allows LRUs to model dependencies across longer time steps while maintaining computational efficiency. One of the most notable advantages of LRUs is their ability to achieve linear complexity in both time and memory, compared to the quadratic complexity of Transformers. This makes LRUs particularly suitable for tasks where sequence length is very large, but computational resources are limited.

The core architecture of LRUs replaces the typical gating functions with a combination of linear dynamics and simple gating, which improves the flow of information across long sequences without the issues traditionally associated with RNNs. LRUs maintain the temporal structure of recurrent neural networks but strip away the unnecessary complexities that limit scalability and gradient propagation. By employing a linear state transition function, they effectively capture long-range dependencies, which is crucial for accurate predictions in time series forecasting.
